Online Sign Identification: Minimization of the Number of Errors in Thresholding Bandits

In the fixed budget thresholding bandit problem, an algorithm sequentially allocates a budgeted number of samples to different distributions. It then predicts whether the mean of each distribution is larger or lower than a given threshold. We introduce a large family of algorithms (containing most existing relevant ones), inspired by the Frank-Wolfe algorithm, and provide a thorough yet generic analysis of their performance. This allowed us to construct new explicit algorithms, for a broad class of problems, whose losses are within a small constant factor of the non-adaptive oracle ones. Quite interestingly, we observed that adaptive methods empirically greatly out-perform non-adaptive oracles, an uncommon behavior in standard online learning settings, such as regret minimization. We explain this surprising phenomenon on an insightful toy problem.

==> other_algorithms.tex <==
% !TeX root = ./neurips_2021.tex
\subsection{Existing algorithms}
\label{sub:existing_algorithms}

We review here existing algorithms for the fixed budget loss minimization problem.

For $L_T = \max_{k\in[K]} E_T^k$, the APT algorithm \cite{locatelli2016optimal}... The bound on the expected loss of APT for that problem gives a bound for the cumulated loss $L_T = \sum_{k\in[K]}a_k E_T^k$ of $\sum_{k\in[K]}a_k \times \text{bound}$ . We recover that bound in our analysis, which is different from the one of \cite{locatelli2016optimal}.

TODO: mention all the APT variants to adapt to the variance of the arms etc.

For $L_T = \sum_{k\in[K]} E_T^k$, the LSA algorithm \cite{tao2019thresholding}...
